Take a deep breath. Benefits of neuroplasticity practices for software developers and computer workers in a family of experiments

Context. Computer workers in general, and software developers specifically, are under a high amount of stress due to continuous deadlines and, often, over-commitment. Objective. This study investigates the effects of a neuroplasticity practice, a specific breathing practice, on the attention awareness, well-being, perceived productivity, and self-efficacy of computer workers. Method. We created a questionnaire mainly from existing, validated scales as entry and exit survey for data points for comparison before and after the intervention. The intervention was a 12-week program with a weekly live session that included a talk on a well-being topic and a facilitated group breathing session. During the intervention period, we solicited one daily journal note and one weekly well-being rating. We replicated the intervention in a similarly structured 8-week program. The data was analyzed using a Bayesian multi-level model for the quantitative part and thematic analysis for the qualitative part. Results. The intervention showed improvements in participants' experienced inner states despite an ongoing pandemic and intense outer circumstances for most. Over the course of the study, we found an improvement in the participants' ratings of how often they found themselves in good spirits as well as in a calm and relaxed state. We also aggregate a large number of deep inner reflections and growth processes that may not have surfaced for the participants without deliberate engagement in such a program. Conclusion. The data indicates usefulness and effectiveness of an intervention for computer workers in terms of increasing well-being and resilience. Everyone needs a way to deliberately relax, unplug, and recover. Breathing practice is a simple way to do so, and the results call for establishing a larger body of work to make this common practice.

==> depr.tex <==
OLD STUFF FROM BIRGIT FIRST ATTEMPT AT TA

\subsubsection{Daily Journal Entries}
The number of answers per subject ranged from one ($1$) to eighty-four ($84$), and so descriptive statistics of the number of code instances are not applicable.

We identified three main types of shares: 1) life occurrence reporting, 2) emotion reporting, and 3) reflections. Often there was a mix of these three types of shares.

\paragraph{1) Life occurrence reporting:} This type of entry would describe what had been happening in the subject's life that day. The most common sub-themes here were work, family, social life, hobbies and pastimes, and health. 

The most frequent theme was work. Here participants talked about remote work and its challenges (more difficult separation between work and private life, inadequate space, disconnectedness), meetings (Zoom fatigue, back-to-back meetings, virtual conferences), deadlines (accumulation, always a next one after), challenges (organisational in circumstances as well as particular project), stress, success, learning experiences, research, etc.

\begin{quote}
    \textit{Once more a busy day, I tried to work hard on finalizing open topics and TODOs, definitely multitasked less and was more focused on the meetings. I tended sometimes to do things in parallel and pay half of the attention to some of the topics in a meeting, that weren’t so relevant to me and my team, but then I just stopped and finalized what was the most important to get ready for one of our Wednesday Meetings. In general a normal day.}
\end{quote}

In family, the answers circled around kids and how to spend time with them, partners and interactions with them, parents and in-laws as well as further relatives, often in relation to health and/or pandemic-related restrictions.

\begin{quote}
    \textit{Today was a good work day. Started with bad news, which took me off my balance. But by the end of it, it was good though: enjoyed teaching, enjoyed my kids, my granny, my parents. I treasure the special  time I had with them. }
\end{quote}

Reports on social life in terms of contact with friends was another frequently addressed topic. There were descriptions of gatherings with friends in new safe-distance ways, whether in online game evenings, joint online cooking sessions, or walks outside (in some cases with masks on).

\begin{quote}
    \textit{I had a good talk with friends today and I feel like that made me relax a bit. I'm still so focused on my studies that It's hard for me to stop up and reflect on things. It is a bit like everything, other than my education, becomes gray and looses taste. I don't have time to stop and settle.}
\end{quote}

Some developed a new hobby or a relived appreciation for old hobbies that got lost due to busyness before the pandemic. There was discovery of new pastimes and ways to spend time in meaningful ways with people in their close circle. 

\begin{quote}
    \textit{Had a wonderful time with my husband, we went and dug out some rosebushes that were given to us for free, put them into our garden- hopefully they like their new place!}
\end{quote}

Furthermore, health frequently came up: 

\begin{quote}
    \textit{"I got my test results as negative but I still was sick. I had fever and anxiety. 
But I slept a lot and had time to reflect over what I need to do in the coming days.
Even with the fever I kept thinking about work."}
\end{quote}

\paragraph{2) Emotion reporting:} This type of entries described the participants emotional experiences in the day and how they had been feeling. Some of the entries only contained a few words, other described experiences in more detail but without the concrete situation. These entries showed a potentially improved self-awareness of the participants over time. Some of them reported to be better in touch with their emotions, realizing when they came up in a specific situation, for example when they got triggered. By noticing such incidents they could take a moment for a deep breath and respond instead of reacting from a place of not being aware. 

This quote reports on the excitement about learning and the emotions brought about by the practice:

\begin{quote}\textit{
    The fact that I am so engaged in learning something new, that also stretches my body in a different way and has a completely new technique, just made me soooo happy. I was present, felt tired but very happy, had a nice and relaxed sleep, and felt very energized.}
\end{quote}

\paragraph{3) Reflections:} The deepest reflective type of entry was when participants took a few steps back to understand the larger picture of what is going on. In these quotes, we see how participants digested the content of the course and how they incorporated the insights in their daily life.
We saw significant gains of insight, which were reflected in the exit interviews for the study.\footnote{The exit interviews are reported on in a different publication for reasons of scope.} 

This quote show reflection on how the participant presents themselves to the world, and that this might not serve them:
\begin{quote}
    \textit{I try to act like I have it all together but I’ve realized the need of letting it go in the past week. That’s perhaps because I have become more conscious about it. }
\end{quote}

This quote reviews the need for doing something to avoid the pure state of 'being':
\begin{quote}
    \textit{It has been difficult sometimes feel not “productive” or connected to work, the sensation and sometimes need to stay connected has reflected while being alone, as long as I listen to, read or watch something I feel at peace, but I find it hard to stay alone in pure silence and disconnected, I noticed that we are not taught to do this at all.}
\end{quote}

This quote reflects on gratitude and appreciation:
\begin{quote}
    \textit{I was thinking today, how even if one’s day went great, one small bad thing can change the perception one has of the entire day. I realized I become thankless of the wonderful day I had because of one sour thing I heard in the evening, or one embarrassing moment that might have occurred in a meeting. I spent time thinking about this and I have decided to try and be more thankful for howsoever my days go and appreciate the good things. }
\end{quote}

This quote understands the term 'mindfulness' on a new level:
\begin{quote}
    \textit{In the past, I always interpreted as the feeling your breath, the air coming in and out, the touch, the noises around you, the texture of the food, etc. As if you had to be still and doing almost nothing to feel physical or some mystical no time/no place sensation. No wonder I was never in the wonderful present moment. During meditation I wondered if that was not it. If it was just being fully dedicated to what we were doing that moment: reading, working, playing, cooking, watching a documentary, etc. Without having your mind often wondering to other places while you do. That is much more useful and attractive. }
\end{quote}

And finally, a reflection on not reporting:

\begin{quote}
    \textit{I have fallen out of reporting for this study, but I have tried to practice what it is teaching. Especially, I have tried to be very present with my grief and not run from it.}
\end{quote}

\subsubsection{Entry / Exit Survey Open Questions}
\todo{@Birgit to describe the qualitative data coding: answers to open questions}

\subsubsection{Analysis of interviews}


%===============================
COPY OF CRISTY*S TEXT JUST IN CASE


\subsection{Qualitative analysis of instruments}

\subsubsection{Demographics}
From 137 sign-ups, 87 converted to completing the entry survey, and 34 completed the study by submitting their exit survey.
The high drop out rates have a number of reasons, which are partially known to the author because of emails kindly sent to her by participants who cared to explain their personal reason for not completing the study. The reasons included the live session being in the middle of get-kids-to-bed time, conflicting commitments for some of the days, and general life stress - which they did note was a good reason to actually do the sessions but they felt they just couldn't at the time.
\todo{use all the email excuses and explanations for why it is not possible even though they know it is good for them.}

\todo{The entry survey showed an age distribution from ...}
 34 completed with participants from 15 countries - India to Ecuador (LIST ALL COUNTRIES HERE because my ego thinks it's cool, and because it increases validity).
 
 
\subsubsection{Thematic analysis}
Coding is the process of labeling and organizing your qualitative data to identify different themes and the relationships between them. Coding qualitative research to find common themes and concepts is part of thematic analysis, which is part of qualitative data analysis. Thematic analysis extracts themes from text~\cite{braun2012thematic}. 
What is common in terms of themes and concepts is not necessarily in and of itself meaningful or important though. 
Thematic analysis includes six phases: 1) Familiarizing oneself with the data, 2) Generating initial codes, 3) Searching for themes, 4) Reviewing potential themes, 5) Defining and naming themes, and 6) Producing the report~\cite{braun2012thematic}.

We present an analysis for the daily journal as well as the entry and exit survey. The weekly survey did not include any open questions.
Table~\ref{tab:codingexample} shows an example of the coding process.

% Table generated by Excel2LaTeX from sheet 'Hoja1'
\begin{table}[htbp]
  \centering
  \caption{Example of the coding process}
    \begin{tabular}{|p{15.215em}|c|p{8.57em}|c|}
    \hline
    \textbf{MEANING UNIT} & \textbf{CODE} & \textbf{THEME} & \textbf{SUB-THEME}\\
    \hline
    \textit{“All together, all the awareness of the program has helped me to be more focused and present, enjoying what I am doing, what I don't enjoy still finalize it without falling in the temptation of getting distracted by the first thing that pops in my mind (still happens, but is getting better)”.} 
    & Focus
    & Perceived changes in participants 
    & At work \\
    \hline
    \end{tabular}%
  \label{tab:codingexample}%
\end{table}%


Regarding qualitative results to answer the six research questions, four themes and four sub-themes were identified presented in the table below.

% Table generated by Excel2LaTeX from sheet 'Hoja1'
\begin{table}[htbp]
  \centering
  \caption{Themes and sub-themes}
    \begin{tabular}{|p{7.5cm}|p{3.5cm}|}
    \hline
    \textbf{Themes} & \textbf{Sub-themes} \\
    \hline
    Main learnings (changes) identified by the participants & \\
    \hline
    Psychological constructs modified during the workshop &\\
    \hline
    Perceived changes in participants & * At work \\
          & * In overall performance \\
    \hline
    Attachment and Integration of techniques in daily life & * Actions \\
          & * Results \\
    \hline
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%

Of course there is much more to be reported, so let's dive in.




\subsubsection{Changes in Mindfulness Attention Awareness}
RQ1: Does the 12-week intervention bring about change in the participants Mindfulness Attention Awareness? \textcolor{red}{Answer: In summary, we ... }

\textcolor{red}{start Cristy description}

\paragraph{Question 1: Main learnings (changes) identified by the participants}
Participants described in their diaries and the interviews how they experienced the changes in perception during the course. They mainly talk about awareness, mindfulness, and attention. They commented how the changes in perception influenced their relationship with themselves, others, and their environment.

\paragraph{Awareness}

\paragraph{} Awareness reported Important changes. The participants mentioned enhanced awareness about themselves, being able to identify better and control feelings and emotions.

\begin{quote}
    \textit{“If I analyze my behaviour before the breathing sessions and now I think that I am more in control of my emotions".
(Participant 3, interview 4)}
\end{quote}

The tools that mainly led the participants to be more aware of their emotions and to being able to control them were analysis and reflection. This participant compared the before and after the course and realized that his control of emotions has increased.

\begin{quote}
    \textit{"I think I became much more aware of feelings, of sensations, and more able to put things aside and seeing the feelings and emotions not being me".
(Participant 14, interview 11)}
\end{quote}

This participant comments that being aware of their emotions has allowed them to separate them from the conception of themselves. Although they do not mention it explicitly, this participant is also integrating learning obtained through the presentations of the exposed topics before beginning the breathing sessions. Module XXXX commented that thoughts are not all that define people.

\begin{quote}\textit{
    "I became more aware of things, and sometimes during practice I’d remember something I had forgotten, and during the meditation I would sometimes become aware that my body and mind became more perceptive...and becoming more aware of pain, but also of my thoughts."
(Participant 15, interview 15)}
\end{quote}

The perceptions went beyond just thoughts and emotions. The previous paragraph shows this participant also perceived physical sensations. It is worth mentioning that memory was another factor that was influenced by breathing practice. 
In addition to self-awareness, some participants also perceived this change concerning their environment.
\begin{quote}
    \textit{“There are lots of wonderful present moments that I am aware of these days”.
(Participant 14, interview 15)}
\end{quote}


\paragraph{Mindfulness}

\paragraph{} Participants have also identified changes in mindfulness. Some were able to recognize and even link them to other thought processes like awareness.
\begin{quote}
    \textit{“I feel more comfortable staying outside of my comfort zone – in the stretch zone, which is what triggers the flow state. So in terms of mindfulness I have been pushed more towards the stretch zone, thanks to the breathing”.
(Participant 2, interview 3)}  
\end{quote}

"The stretch zone" is how this participant identifies the experience of being outside the comfort zone and the flow state. They also mentioned that they felt pushed towards that area after having practiced the breathing exercises. The stretch zone is where they feel comfortable. 
\begin{quote}
    \textit{“There are things I have no control on. When this things happen it is hard to concentrate on what I am doing. but reminding what is important at this moment and breathing is helping me recently to get my thought together”.
(participant 1, journal)}    
\end{quote}

The previous paragraph illustrates how a participant, focused on mindfulness added to the breathing practice, manages to focus and organize their thoughts. The participant can also identify what makes it difficult for them to manage their concentration, which implies a process of awareness. 
\begin{quote}
    \textit{“In reflection, lots of similar experiences in the past were less pleasant, due to my lack of self awareness and poor mindfulness which allowed me to defuse disruptive behaviours triggered by stress (e.g., loosing focus, feeling insecure, cognitive overload, etc.)”.
(participant 2, journal)}   
\end{quote}

This participant even compared how they lived their past experiences in a different state of awareness and mindfulness and concluded that stress was the reason for those behaviors. They also identified their emotions and behaviors. Likewise, they mentions that it was thanks to the reflection that they managed to have this insight after participating in the breathing course.

\paragraph{Attention}

\paragraph{}Finally, attention was also influenced in the participants. Mainly link to personal internal processes instead of working or studying.
\begin{quote}
    \textit{“And with your lessons I started giving more attention to the things that I knew were more important to me, and now I do that”. 
(Participant 6, interview 1)}    
\end{quote}

This participant mentions that they already knew the things that are important to them. However, it was after the course that they did insight and began to deal with them. In addition to the attention process, this participant also had a change in awareness. They became aware that they needed to pay attention to those important things. They do now, and they are aware of that change. 
\begin{quote}
  \textit{“For me, the course was closely linked to high corona numbers and was a good instrument to let go and concentrate on myself - and what the constant checking of numbers does to me, to my attention”.
(Participant 16, interview 14)}  
\end{quote}

In this case, the participant shifted their focus from the environment around them to themselves. They write that they used as an instrument what they learned in the course to "let go" of the issues related to the pandemic and redirect their attention to themselves.

The excerpts of the interviews and the daily journal show that the participants carry out more than one thought process at the same time. Sometimes they are not aware of the combination of these processes. However, when describing how their experiences are, the combination of attention, awareness, and in some cases, also mindfulness is clear. Similarly, most of the participants' insights happened through reflection, which was motivated by writing every day. Keeping a journal pushed participants to grade their day and dig deeper into what was most important to them.

\textcolor{red}{end Cristy description}
